Yacc is dead

We present two novel approaches to parsing context-free languages. The first approach is based on an extension of Brzozowski's derivative from regular expressions to context-free grammars. The second approach is based on a generalization of the derivative to parser combinators. The payoff of these techniques is a small (less than 250 lines of code), easy-to-implement parsing library capable of parsing arbitrary context-free grammars into lazy parse forests. Implementations for both Scala and Haskell are provided. Preliminary experiments with S-Expressions parsed millions of tokens per second, which suggests this technique is efficient enough for use in practice.

==> abstract.tex <==
% Derivatives (also known as the left quotient) of formal languages are
% have been used for linguistic analysis since at least Brzozowski's
% work on regular languages in the 1960s.
% %
% Out of fashion in the mainstream parsing community for almost equally as long, 


We present two novel approaches to parsing context-free languages.
The first approach is based on an extension of Brzozowski's derivative
from regular expressions to context-free grammars.  The second
approach is based on a generalization of the derivative to parser
combinators.  The payoff of these techniques is a small (less than 250
lines of code), easy-to-implement parsing library capable of parsing
arbitrary context-free grammars into lazy parse forests.
Implementations for both Scala and Haskell are provided.  Preliminary
experiments with S-Expressions parsed millions of tokens per second,
which suggests this technique is efficient enough for use in practice.

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "paper-sigplan.tex"
%%% End: 



==> local-macros.tex <==
 


==> meta.tex <==

\newcommand{\mylongtitle}{Yacc is dead}
\newcommand{\mysubtitle}{Practical parsing with derivatives}
\newcommand{\myshorttitle}{Yacc is dead}
\newcommand{\mytitle}{Yacc is dead}


% Tweakable
\newcommand{\mytitlebanner}{In submission}
\newcommand{\footertitle}{\myshorttitle}
